Optics for Premonoidal Categories

We further the theory of optics or "circuits-with-holes" to encompass premonoidal categories: monoidal categories without the interchange law. Every premonoidal category gives rise to an effectful category (i.e. a generalised Freyd-category) given by the embedding of the monoidal subcategory of central morphisms. We introduce "pro-effectful" categories and show that optics for premonoidal categories exhibit this structure. Pro-effectful categories are the non-representable versions of effectful categories, akin to the generalisation of monoidal to promonoidal categories. We extend a classical result of Day to this setting, showing an equivalence between pro-effectful structures on a category and effectful structures on its free tight cocompletion. We also demonstrate that pro-effectful categories are equivalent to prostrong promonads.

==> eptcsdata.tex <==
\providecommand{\firstpage}{152}
\providecommand{\publicationstatus}{S. Staton, C. Vasilakopoulou (Eds.):\\
Applied Category Theory 2023 (ACT2023)\\
EPTCS 397, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.397.10}{10.4204/EPTCS.397.10}}
\pdfoutput=1

